Prophet Secretary and Matching: the Significance of the Largest Item

The prophet secretary problem is a combination of the prophet inequality and the secretary problem, where elements are drawn from known independent distributions and arrive in uniformly random order. In this work, we design 1) a $0.688$-competitive algorithm, that breaks the $0.675$ barrier of blind strategies (Correa, Saona, Ziliotto, 2021), and 2) a $0.641$-competitive algorithm for the prophet secretary matching problem, that breaks the $1-1/e\approx 0.632$ barrier for the first time. Our second result also applies to the query-commit model of weighted stochastic matching and improves the state-of-the-art ratio (Derakhshan and Farhadi, 2023).

==> app-decreasing-0.694.tex <==
\section{Decreasing Results}
\label{app:decreasing}

\begin{lemma}
$f(h)=\frac{1 - e^{-h \threshold}}{h}$ and $g(h)=\frac{e^{-h \threshold} - e^{-(2-h) + (2-2h) \threshold}}{2-h}$ are decreasing in $h$ when $0<h<1-\ln 2$ for $\beta\approx 0.367$.
\end{lemma}

\begin{proof}
Note that $f(h)$ can be viewed as the slope of the line connecting the points $(0,1)$ and $(h, e^{-h \threshold})$ on the curve $y = e^{-x \threshold}$. Since function $y=e^{-x\threshold}$ is convex for $0<\threshold<1$, the slope of the line segment is decreasing in $h$.

For $g(h)$, we first calculate its derivative over $h$:
\[
    g'(h)=\frac{e^{-2 \beta h-2+2\beta+h}\left(e^{\beta h+2-2\beta-h}(\beta(h-2)+1)+(4 \beta-2 \beta h+h-3)\right)}{(h-2)^2}
\]
Then, denote $l(h)=e^{\beta h+2-2\beta-h}(\beta(h-2)+1)+4 \beta-2 \beta h+h-3$, we have:
\[
    l'(h)=e^{\beta h+2-2\beta-h}(\beta(\beta-1)h-2\beta^2+4\beta-1)-2\beta+1
\]
Note that $1-2\beta>0$ and $\beta(\beta-1)h-2\beta^2+4\beta-1\geq \beta (\beta-1)(1-\ln 2) - 2\beta^2 + 4\beta - 1 =  (-1-\ln 2) \beta^2 + (3+\ln 2) \beta - 1 \approx 0.1273>0$ for $\beta\approx 0.367$. Thus, $l'(h)>0$  for any $h\in (0,1-\ln 2)$. Therefore, $l(h)\leq l(1-\ln 2)=e^{\beta(-1-\ln 2)+1+\ln 2} (\beta(-1-\ln 2)+1) \approx -0.345 < 0$ for any $h\in (0,1-\ln 2)$. Thus, $g'(h)=\frac{e^{-2 \beta h-2+2\beta+h} }{(h-2)^2} l(h)
<0$ for any $h\in (0,1-\ln 2)$. Thus, $g(h)$ is decreasing in $h$ for $0<h<1-\ln 2$, which completes the proof.
\end{proof}

==> intro_backup.tex <==
The study of prophet inequality dates back to 1970s~\cite{krengel1977semiamarts,krengel1978} in optimal stopping theory. Consider $n$ boxes with independent random values arrive one by one in an adversarial order. The value distribution $F_i$ of each box $i$ is known upfront to the algorithm, but the realization $v_i \sim F_i$ is only revealed on its arrival. After seeing the identity $i$ of the box and its associated value $v_i$, the algorithm decides immediately whether to select the box: if the algorithm selects $i$, it collects a value of $v_i$ and the game ends; otherwise, it continues to the next box. The goal is to maximize the expected value of the selected box and compete against the prophet, i.e., the expected maximum value $\Ex{\max_i v_i}$. It is shown that the optimal competitive ratio is $\frac{1}{2}$ for this problem.

A fundamental extension of the prophet inequality is prophet matching. Consider an underlying bipartite graph with edge weights drawn from known distributions. One side of the vertices are known upfront and the other side of vertices arrive online. Upon the arrival of a vertex $v_i$, the weight of its incident edges are revealed and the algorithm decides whether to match $v_i$ and to which offline vertex. The classic prophet inequality is captured by this model with one offline vertex. Feldman, Gravin, and Lucier~\cite{soda/FeldmanGL15} established a tight $\frac{1}{2}$ competitive algorithm for the matching setting, and their result is further generalized to settings when all vertices arrive online~\cite{mor/EzraFGT22}.

In this work, we concern the secretary variants (aka. random order variant) of prophet inequality and prophet matching, i.e., the setting when boxes (resp. vertices) arrive in uniformly random order.

The study of prophet secretary is initiated by Esfandiari et al.~\cite{esa/EsfandiariHLM15}, who designed a $1-1/e \approx 0.632$ competitive algorithm and provided an upper bound of $0.75$\footnote{The competitive ratio of an algorithm is a number between $[0,1]$. A lower bound corresponds to an algorithm and an upper bound corresponds to an impossibility result.}. 
% Later, the same ratio has been reproduced by Correa et al.~\cite{??} through a nonadaptive algorithm and by Ehsani et al.~\cite{??} through a single-threshold algorithm.
Since then, a sequence of follow-up work~\cite{ec/AzarCK18, mp/CorreaSZ21, corr/Harb23, ec/BubnaC23, corr/Giambartolomei23} has been focused on closing the gaps. The state-of-the-art lower and upper bounds are $0.672$ by Harb~\cite{corr/Harb23} and $0.723$ by Giambartolomei et al.~\cite{corr/Giambartolomei23} respectively.

Less progress is made on the prophet secretary matching problem since the $1-1/e$ competitive algorithm by Ehsani et al.~\cite{soda/EhsaniHKS18}.
Indeed, it is only very recently the $1-1/e$ barrier gets surpassed in two special cases, namely 1) the i.i.d. setting studied by Yan~\cite{soda/Yan24} and Qiu et al.~\cite{wine/QiuFZW23}; and 2) the query-commit setting studied by Derakhshan and Farhadi~\cite{soda/Derakhshan023}. Beating $1-1/e$ for prophet secretary matching remains one of the most intriguing open questions in the online algorithms community.

\subsection{Our Contributions}
We improve the state-of-the-art competitive ratios of prophet secretary, and matching. 
\begin{itemize}
\item We design a $0.688$-competitive algorithm for the prophet secretary problem. Besides the straightforward numerical improvement\footnote{We remark that the latest improvement prior to our work is from $0.669$~\cite{mp/CorreaSZ21} to $0.672$~\cite{corr/Harb23}. We argue that our numerical improvement is significant.}, our result surpasses the $0.675$ barrier of \emph{blind strategies}~\cite{mp/CorreaSZ21}, the family of algorithms that Correa et al.~\cite{mp/CorreaSZ21} and Harb~\cite{corr/Harb23} focused on. Conceptually, our result asserts that the detailed stochastic information of the underlying distributions are crucial for the prophet secretary problem. In contrast, blind strategies only utilize the distribution of the maximum value. Though not surprising, it is technically challenging to incorporate such information into algorithm design and analysis.
\item We design a $0.641$-competitive algorithm for the prophet secretary matching problem, breaking the $1-1/e$ barrier for the first time. As an implication, we also improve the state-of-the-art ratio of the query-commit setting from $0.633$~\cite{soda/Derakhshan023} to $0.641$ through folklore reductions from the query-commit model to the secretary model.
\end{itemize}

\paragraph{Our Techniques.}
As mentioned earlier, an important special case of the prophet secretary (matching) problem is the i.i.d. setting, when every box (vertex) is associated with the same distribution.
% so that all arrival orders are the same. 
The i.i.d. prophet inequality is shown to have an optimal competitive ratio of $0.745$\footnote{The unique solution to $\int_0^1 \frac{1}{y(1-\ln y)+1/\Gamma-1}\dd y=1$.} after a long time of research~\cite{hill1982,stoc/AbolhassaniEEHK17,mor/CorreaFHOV21}; and the i.i.d. prophet matching problem is shown to have a competitive ratio of $0.645$ by Yan~\cite{soda/Yan24}.

Our starting point is two subroutines that generalize algorithms from i.i.d. instances to arbitrary infinitesimal instances. Informally, an instance is infinitesimal if each box (resp. vertex) contributes negligibly to the prophet. This assumption is naturally satisfied by symmetry for i.i.d. instances. 

\begin{itemize}
\item For the prophet secretary problem, similar algorithms are designed by Abolhassani et al.~\cite{stoc/AbolhassaniEEHK17} and Liu et al.~\cite{ec/LiuLPSS21}. They proved that if either 1) every distribution appears sufficiently many times~\cite{stoc/AbolhassaniEEHK17, ec/LiuLPSS21} or 2) every distribution has only a negligible probability of being non-zero~\cite{ec/LiuLPSS21}, then there exists a $0.745$-competitive algorithm. 

Nevertheless, a separation is shown between the i.i.d. setting and the secretary setting. And the existing hard instances for the prophet secretary problem~\cite{mp/CorreaSZ21,ec/BubnaC23,corr/Giambartolomei23} share the same structure of a large (non-infinitesimal) box plus $n$ infinitesimal i.i.d. boxes. 
Inspired by these hard instances, our modified algorithm includes an ad hoc and instance-wise design for the largest box, and then treats the other boxes as if they were infinitesimal. Our algorithm jumps out of the family of blind strategies in the most obvious way, as a blind strategy cannot even differentiate the largest box from others, but it turns out to be powerful.
\zhihao{It is a bit inaccurate to say so, since we actually only do a two-stage algorithm, rather than the continuous $0.745$ algorithm.} 

\item For the prophet secretary matching problem, it is less trivial to generalize existing algorithms from the i.i.d. setting. Specifically, the algorithms of Yan~\cite{soda/Yan24} and Qiu et al.~\cite{wine/QiuFZW23} rely heavily on a preprocessing step that is tailored for i.i.d. instances. Our subroutine crucially avoids this step while maintaining necessary properties for achieving the same competitive ratio $0.645$ for infinitesimal instances. On the other hand, the worst-case competitive ratio of this subroutine can be as bad as $1-1/e$ if each offline vertex is associated with an important online neighbor. 
To complement this scenario, we introduce a variant of the random order contention resolution scheme algorithm for matching~\cite{esa/LeeS18,icalp/FuTWWZ21} and then randomize it with the subroutine. We show that our hybrid algorithm achieves the stated $0.641$ competitive ratio.
\end{itemize}

\subsection{Related Works}

\begin{itemize}
\item order selection
\item combinatorial settings beyond matching: Besides matching, the prophet inequality has been generalized to online stochastic selection problems under combinatorial feasibility constraints, including matroids~\cite{geb/KleinbergW19}, combinatorial auctions~\cite{soda/FeldmanGL15, siamcomp/DuttingFKL20}, and general downward-closed constraints~\cite{stoc/Rubinstein16}.

\item unweighted / vertex-weighted online stochastic matching
\end{itemize}


==> prelim.tex <==
\section{Preliminaries}
\zhihao{Some general comments: 
\begin{itemize}
    \item I have defined macros for Probability / Expectation / Indicator function. Please follow.
    \item The format of the references are not standard. Please use the bibtex from dblp.
\end{itemize}}


\subsection{Prophet Secretary Matching}

Let there be an edge-weighted bipartite type graph $G=(U,V,E,w)$.
Here, $U$ is to the set of offline vertices that are known in advance to the algorithm, $V$ is to the set of all possible types of online vertices.
Further, $E$ denotes the set of edges, and $w : E \to [0, +\infty)$ denotes the edge-weights.
That is, $w_{uv}$ is weight of edge $(u, v) \in E$.

There are $n$ online vertices.
Online vertex $1 \le i \le n$ has a type $v_i \in V$ drawn independently from a known distribution $F_i$, and an arrival time $t_i$ drawn independently and uniformly from $[0,1]$.
We use $\piv$ to denote the probability of $v_i = v$.
When online vertex $i$ arrives at time $t_i$, the algorithm sees its index $i$, type $v_i$, and arrival time $t_i$, and must decides how to match this online vertex immediately.
The goal is to maximize the total weight of the edges in the matching.

We will compare to the offline optimal matching.
An online algorithm is $\Gamma$-competitive if the expected total weight of its matching is at least a $\Gamma$ fraction of the expectation of the maximum total weight given by the offline optimal matching.

We remark that the Prophet Secretary problem is a special case of Prophet Secretary Matching when there is only one offline vertex.

% and to compete against the expected maximum matching.


%\zhihao{You might want to use the materials in Section 4.1.}
%As a natural generalization of the Prophet Secretary problem, we consider the following matching problem. 

%Suppose there is an edge-weighted bipartite graph $G=(U,V,E)$, where $U$ and $V$ are the two disjoint sets of vertices, and $E$ is the set of edges. Each vertex in $U$ is called an offline vertex, and each vertex in $V$ is called an online vertex. The weight of an edge $(u,v)$ is denoted by $w_{uv}$. During the matching process, each online vertex $v$ arrives at a time $t_v$ drawn i.i.d. from $U[0,1]$, and the player should immediately decide whether to match $v$ to an offline vertex $u$ or not. If the player decides to match $v$ to $u$, he gets value $w_{uv}$. The goal is to maximize the expected value of the matching.

%\subsection{Notations}
%
%For the discrete random variables $v_i$'s, we use $p_i^v$ to denote the probability that the value of item $i$ is $v$.
%
%\begin{itemize}
%\item Matching
%\begin{itemize}
%\item $t_i \in [0,1]$ arrival time of box/vertex $i$ 
%\item Type graph: $G=(U,V,E)$, edge $(u,v)$ with weight $w_{uv}$, $U$ for offline and $V$ for online
%\item $v_i \in V$ drawn from $F_i$
%\item $p^v_i$: probability of $v_i = v$
%\item $x_i^{(u,v)}$: probability of matching $i$ to $u$ and $v_i = v$
%\item $\rho = x/p$: density
%\item $g_i^{(u,v)}(t)= a^{uv}_i(t) \cdot \exp(-\int_0^t A_i^u(y) dy)$
%\item $a$ for active rate, $A^u_i(t) = E_{v}[a_i^{uv}(t)]$
%\item $a^{uv}_i(t)$ depends on three parameteres: $s=2$, $\beta_1,\beta_2$
%\end{itemize}
%\end{itemize}


==> temp.tex <==

The algorithm is as follows:
\begin{algorithm}[H]
\caption{step activation}
\label{algo:step-act-rate-0.688}
\begin{algorithmic}[1]
    \State Calculate
    $i_0=\arg \max_i \sum_v x_i^v, \quad x_0 = \sum_v x_{i_0}^v$
    \State Select an $s>1$, calculate $z_{i_0}^v = \frac{1}{s-1} (s\rho_{i_0}^v - 1)^+$ and $h_0 = \sum_{v} p_{i_0}^v z_{i_0}^v$.
    \State Select $z_i^v$'s for all $i\neq i_0$, satisfying that $\sum_{i\neq i_0} \sum_v p_i^v z_i^v = \min\{h_s(x_0) - h_0, 1 - x_0\}\triangleq h_{ot}$, and $z_i^v \in [\frac{1}{s-1}(s\rho_i^v - 1)^+, \rho_i^v]$. (Function $h_s$ is defined in \Cref{app:h-function})
    \State Select $t_0\leq t_1\leq t_2$.
    \For{Time $t$ from $0$ to $1$}
    \State Upon the arrival of box $i=i_0$ at time $t$ with value $v$:
    \State Activate it with activation probability $g_{i_0}^v(t)$, where $g_{i_0}^v(t)$ is defined as follows.
    \[
        g_{i_0}^v(t)=\left\{ \begin{aligned}
            0 & \quad \text{if } t\in [0,t_0],\\
            z_{i_0}^v & \quad \text{if } t\in [t_0, t_2],\\
            s\rho_{i_0}^v - (s-1) z_{i_0}^v & \quad \text{if } t\in [t_2, 1].
        \end{aligned} \right.
    \]
    \State Upon the arrival of box $i\neq i_0$ at time $t$ with value $v$:
    \State Activate it with activation rate $a_i^v(t)$, namely with activation probability $g_i^v(t) = a_i^v(t)e^{-\int_0^t A_i(x)dx}$, where $a_i^v(t)$ is defined as follows:
    \[
        a_i^v(t)=\left\{ \begin{aligned}
            z_i^v & \quad \text{if } t\in [0,t_1],\\
            s\rho_i^v - (s-1) z_i^v & \quad \text{if } t\in [t_1, 1].
        \end{aligned} \right.
    \]
    \State Accept the box $i$ if it is the first activated box.
    \EndFor
    \end{algorithmic}
\end{algorithm}

\begin{theorem}
    \Cref{algo:step-act-rate-0.688} is $0.688$-competitive.
\end{theorem}

% The proof of this theorem is a little complicated, and we will give a sketch of the proof in the following. The detailed proof can be found in the appendix.

\begin{proof}
    At first, we show the algorithm is correct.

    \begin{itemize}
        \item For any $s$, $z_i^v$ can be found satisfying the constraints.\\
        Note that $\frac{1}{s-1}(s\rho_i^v - 1)^+ \leq \rho_i^v$, it suffices to show that 
        \[
            \sum_{i\neq i_0} \sum_v p_i^v \frac{1}{s-1} (s\rho_i^v - 1)^+ \leq \min\{h_s(x_0) - h_0, 1 - x_0\} \leq \sum_{i\neq i_0} \sum_v p_i^v \rho_i^v.
        \] \\
        Note that we have $\sum_{i\neq i_0} \sum_v p_i^v \rho_i^v =\sum_{i\neq i_0} \sum_v x_i^v = 1 - x_0$, and according to the definition of $h_s(x)$ in~\cref{app:h-function}, we have:
        \[
            \begin{aligned}
                &\sum_{i\neq i_0} \sum_v \frac{1}{s-1} p_i^v (s\rho_i^v - 1)^+ = \sum_{i\neq i_0} \sum_v \frac{1}{s-1} (sx_i^v - p_i^v)^+ \\
                =& \sum_{i} \sum_v \frac{1}{s-1} (sx_i^v - p_i^v)^+ -h_0  \leq h_s(x_0) - h_0.
            \end{aligned}
        \]
        These complete the proof.
        \item The activation probability is well-defined.\\
        Recall that for any $i$, $0\leq x_i^v \leq \rho_{i}^v\leq 1$. \\
        For $g_{i_0}^v(t)$: obviously $z_{i_0}^v\geq 0$, $z_{i_0}^v \leq \rho_{i_0}^v\leq 1$, $s \rho_{i_0}^v - (s-1) z_{i_0}^v= s \rho_{i_0}^v - (s \rho_{i_0}^v - 1)^+ = \min\{s \rho_{i_0}^v, 1\}\in [0,1]$, thus $g_{i_0}^v(t)$is well-defined.\\
        For $g_i^v(t)$ that $i\neq i_0$: obviously $z_i^v\in [0,1]$, $s \rho_i^v - (s-1) z_i^v \in [\rho_i^v, \min\{s \rho_i^v, 1\}]\subset [0,1]$, thus $a_i^v(t)\in [0,1]$, and $g_i^v(t)\leq a_i^v(t)$ is well-defined.
    \end{itemize}

    Then, we show the competitive ratio of the algorithm.
    
    Actually, we do not give the explicit form of $s$, $t_0,t_1,t_2$. We only show that there \emph{exists} an algorithm in this form that is $0.688$-competitive. The idea is to express the competitive ratio of the algorithm as a function $\Gamma$ of $s$, $t_0,t_1,t_2$, then use computer to verify that:
    $S=\{2 + 0.1 n  \:| n\in \mathbb{N},~ n\le 12\}$ we have:
    \[
        \forall 0\le x_0\le 1, \exists s\in S, \forall 0\le h_0\le x_0, \exists 0\le t_0\le t_1\le t_2\le 1, \Gamma(s, x_0, h_0, t_0, t_1, t_2) > 0.688.
    \]

    By \Cref{lemma:single-act-rate}, the probability that the box $i(\neq i_0)$ was not activated before time $t$ is: 
    \[1-\sum_v p_i^v\int_0^t g_i^v(t) \dif t = \exp\left(-\int_0^t A_i(y)\dif y\right),\]
    where $A_i(t)$ equals $\sum_v p_i^v z_i^v$ when $t\in [0, t_1]$ and equals $sx_i - \sum_v p_i^v z_i^v$ otherwise.
    \ldcsays{unify the exp or $e^{..}$?}

    Hence the probability of not existing any box $i\neq i_0$ was activated before time $t$ is:
    \[
    \begin{aligned}
        K(t)\triangleq  & \prod_{i\neq i_0} \exp\left(-\int_0^t A_i(y)\dif y\right) 
        = \exp\left(-\int_0^t \sum_{i\neq i_0}A_i(y)\dif y\right)\\ 
        = &\exp\left(-h_{ot}\cdot t - s(1 - x_0 - h_{ot}) \cdot (t - t_1)^+\right),
    \end{aligned}    
    \]
    since $\sum_{i\neq i_0}A_i(t)$ equals $ h_{ot}$ for $t\in [0, t_1]$ and equals $s(1 - x_0) - (s-1)\cdot h_{ot}$ for $t\in [t_1, 1]$. 
    % For simplicity, we also denote $h_{ot}\cdot t + s(1 - x_0 - h_{ot}) \cdot (t - t_1)^+$ by $K(t)$.

    The probability of box $i_0$ was not activated before time $t$ is 
    \[
        \begin{aligned}
            L(t) \triangleq & 1 - \sum_v p_{i_0}^v \int_0^t g_{i_0}^v(x) \dif x = 1 - h_0 \cdot (t - t_0)^+ - s (x - h_0) \cdot (t - t_2)^+,
        \end{aligned}
    \]
    since $\sum_v p_{i_0}^v g_{i_0}^v(t)$ equals $0$ for $t\in [0, t_0]$ and equals $h_0$ for $t\in [t_0, t_2]$ and equals $sx_0 - (s-1)h_0$ for $t\in [t_2, 1]$.
    %  For simplicity, we denote $h_0 \cdot (t - t_0)^+ + s (x - h_0) \cdot (t - t_2)^+$ by $L(t)$.

    Now we are ready to competitive analysis.

The probability of box $i_0$ is accepted with value $v_{i_0} = v$ is:

\begin{align*}
    & \int_0^1 g_{i_0}^v(t) \exp\left(-K(t)\right) \dif t \\
    = ~ & z_{i_0}^v \int_{t_0}^1 \exp\left(-K(t) \right)\dif t + (\rho_{i_0}^v - z_{i_0}^v) \cdot s \int_{t_2}^1 \exp\left(-K(t) \right) \dif t \\
    \ge ~ & \rho_{i_0}^v \cdot \min\{\int_{t_0}^1 \exp\left(-K(t) \right)\dif t,
    ~ s \int_{t_2}^1 \exp\left(-K(t) \right) \dif t\}
\end{align*}

The probability of box $i\neq i_0$ is chosen conditioned on $v_i = v$ is:
\begin{align*}
    & \int_0^1 g_i^v(t) \cdot \left(1 - h_0 \cdot (t - t_0)^+ - s (x - h) \cdot (t - t_2)^+\right) \cdot \prod_{i'\neq i, i_0} \exp\left(-\int_0^t A_{i'}(y)\dif y\right) \dif t \\
    = ~ & \int_0^1 a_i^v(t) \cdot  \prod_{i'\neq i_0} \exp\left(-\int_0^t A_{i'}(y)\dif y\right) \cdot \left(1 - L(t)\right) \dif t \\
    = ~ & \int_0^1 a_i^v(t) \cdot \exp\left(-K(t) \right) \cdot \left(1 - L(t)\right) \dif t \\
    = ~ & z_i^v \cdot \int_0^1 \exp\left(-K(t) \right) \cdot \left(1 - L(t)\right) \dif t +  (\rho_i^v-z_i^v) \cdot s \int_{t_1}^1 \exp\left(-K(t) \right) \cdot \left(1 - L(t)\right) \dif t\\
    \ge ~ & \min\{\int_0^1 \exp\left(-K(t) \right) \cdot \left(1 - L(t)\right) \dif t,
    ~ s\cdot  \int_{t_1}^1 \exp\left(-K(t) \right) \cdot \left(1 - L(t)\right) \dif t\}
\end{align*}

Therefore, the algorithm is $\Gamma$-competitive for:
\begin{align}
    \Gamma := \min \{& \int_{t_0}^1 \exp\left(-K(t) \right)\dif t,
    ~ s\cdot \int_{t_2}^1 \exp\left(-K(t) \right) \dif t,\\
    & \int_0^1 \exp\left(-K(t) \right) \cdot \left(1 - L(t)\right) \dif t,
~ s\cdot  \int_{t_1}^1 \exp\left(-K(t) \right) \cdot \left(1 - L(t)\right) \dif t \}
\end{align}
which is a function with respect to $s, x_0, h_0, t_0, t_1, t_2$.

We use computer numerically verify that for $S=\{2 + 0.1 n  \:| n\in \mathbb{N},~ n\le 12\}$ we have:
\[\forall 0\le x_0\le 1, \exists s\in S, \forall 0\le h_0\le x_0, \exists 0\le t_0\le t_1\le t_2\le 1, \Gamma(s, x_0, h_0, t_0, t_1, t_2) > 0.688.\]

% \[\int_0^1 k_{ij}(t) e^{-\sum_{i}Z_i(t)}\dif t = \frac{1}{s-1}(s\rho_{ij}-1)^+\cdot \int_0^1 + s\left(\rho_{ij}-\frac{1}{s-1}(s\rho_{ij}-1)^+\right)\cdot \int_{\alpha}^1\ge \Gamma\rho_{ij}\]

% \[\int_0^{1}e^{-Z}dt,~s\cdot\int_{\alpha}^1 e^{-Z}dt\ge \Gamma.\]

% \[\sum_{ij}\frac{1}{s-1}(sx_{ij}-p_{ij})^+\le 1 - \frac{\ln s}{s-1} + c\cdot \max_{i} \sum_j x_{ij}\]

% $\sum_{i}\frac{1}{s-1}(sx_i-p_i)$ is maximized at $p_i = \frac{x_i}{1-\sum_{j<i}x_i}$. Further, this is maximized at $(x_0,x_1\cdots) = (x, x\cdots)$ when $x_i$ are upper bounded by $x$. We denote this maximized value by $h(x)$.

% Competitive ratio for box $i$:

% \[\prod_{i'} e^{-Z_i'(t)} = \exp\Big(-h(x) - s\cdot (t-\alpha)^+ (1-h(x))\Big)\]

% \[\prod_{i'\neq i} e^{-Z_i'(t)} = \exp\Big(-(h(x) - h) - s\cdot (t-\alpha)^+ (1-x-h(x)+h)\Big)\]
% \[R_1 = \int_\beta^1 \exp(\cdots) dt\]
% \[R_2 = s\cdot\int_\gamma^1 \exp(\cdots) dt\]

% Competitive ratio for other boxes:
% \[R_3 = \int_0^1 \exp(\cdots)\cdot \Big(1 - (t-\beta)^+\cdot h - s \cdot 1\{t>\gamma\}(x - h)\Big) dt\]
% \[R_4 = s\cdot \int_\alpha^1 \exp(\cdots)\cdot \Big(1 - (t-\beta)^+\cdot h - s \cdot 1\{t>\gamma\}(x - h)\Big) dt\]

% Competitive ratio $R = \min\{R_1, R_2, R_3, R_4\}$

\end{proof}
